PDNPulse: Sensing PCB Anomaly with the Intrinsic Power Delivery Network

The ubiquitous presence of printed circuit boards (PCBs) in modern electronic systems and embedded devices makes their integrity a top security concern. To take advantage of the economies of scale, today's PCB design and manufacturing are often performed by suppliers around the globe, exposing them to many security vulnerabilities along the segmented PCB supply chain. Moreover, the increasing complexity of the PCB designs also leaves ample room for numerous sneaky board-level attacks to be implemented throughout each stage of a PCB's lifetime, threatening many electronic devices. In this paper, we propose PDNPulse, a power delivery network (PDN) based PCB anomaly detection framework that can identify a wide spectrum of board-level malicious modifications. PDNPulse leverages the fact that the PDN's characteristics are inevitably affected by modifications to the PCB, no matter how minuscule. By detecting changes to the PDN impedance profile and using the Frechet distance-based anomaly detection algorithms, PDNPulse can robustly and successfully discern malicious modifications across the system. Using PDNPulse, we conduct extensive experiments on seven commercial-off-the-shelf PCBs, covering different design scales, different threat models, and seven different anomaly types. The results confirm that PDNPulse creates an effective security asymmetry between attack and defense.

==> doc/crossboard_detection.tex <==
We also test the feasibility of in-field detection by plugging the network adapter into the MSI H310M PRO-VDH PLUS computer motherboard. The probe is attached to the PCI-E pins on the motherboard.
Fig.\ref{fig:network_adapter_results}(b) shows the $Z_{11}$ measured from the PCI-E power pins on the motherboard, where the impedance profiles of all boards are plotted.
The blue and red lines represent genuine boards and suspicious ones, respectively, and the green line shows the $Z_{11}$ when no board is connected to the PCI-E. 
Besides the PDN of the network adapter, the measured impedance profiles (blue and red lines) are also distorted by the PDN of the motherboard and the parasitics of PCI-E connector.
Under the distortion, we are still able to identify the suspicious boards.
This preliminary result illustrates one advantage of the PDN-based method, that is, it does not require removing the boards from the server/motherboard, thus facilitating remote anomaly detection. 

==> doc/setup.tex <==


Fig.\ref{fig:setup}(a) shows the experimental setup for measuring the PCB PDN impedance profiles throughout this paper.
We utilize the Keysight E5063A VNA to measure $S21$ and take frequency domain $300KHz\sim 3GHz$ as the band of interest.
The VNA is configured to 2-port shunt-through method for small impedance measurements as introduced in section ~\ref{sec:pdn_measure}.
We set the VNA to use $10KHz$ maximum IF bandwidth and collect 1024 points for each impedance profile. 
In addition, the positioners and liftable platform are adapted to increase the measurement stability and efficiency.
Before the measurements, the standard 2-port calibration is performed to correct the errors caused by the coaxial cables and etc.
And for each measurement, the conversion from S-parameters to Z-parameters is performed according to Equation~\ref{eq:s2z} and~\ref{eq:s2z_matrix}.
Note that for all experiments in this work, the PDN impedance profile is measured off-line and the boards are powered off. 

When performing the measurements, the PCB PDN can be connected to VNA either directly through coaxial cables or aided by the probes.
The former configuration can provide the most stable and accurate results.
However, this configuration can only support PCBs embedded with coaxial adapters, which are rarely included in commercial designs.
To relief this limitation, in this paper, an easy-to-use probe is developed to facilitate real-world measurements, as shown in Fig.\ref{fig:setup}(b).
The probe is specifically designed for small impedance measurements and two probe tips (for signal and ground respectively) with springs are connected to a coaxial adapter that can be further connected to VNA through the cable.
In addition, a mechanical probe tuner (the yellow part of Fig.\ref{fig:setup}(b)) is designed to precisely adjust the space between the probe tips.
Compared with expensive high specification commercial probes with fixed tip space, our probe is proved to achieve a good trade-off among cost, error\footnote{Our probe introduces a consistent systemic error to all the measurements due to the parasitic effects of the probe, which however, won't affect the findings from the results. This error can be further removed if calibration is conducted at the probe tip end.}, and easy-of-use. 
In this paper, without specifically mentioning, we adapt this experimental setup combined with the designed probe for PCB anomaly detection. 


